Multi-Label Quantification

Quantification, variously called "supervised prevalence estimation" or "learning to quantify", is the supervised learning task of generating predictors of the relative frequencies (a.k.a. "prevalence values") of the classes of interest in unlabelled data samples. While many quantification methods have been proposed in the past for binary problems and, to a lesser extent, single-label multiclass problems, the multi-label setting (i.e., the scenario in which the classes of interest are not mutually exclusive) remains by and large unexplored. A straightforward solution to the multi-label quantification problem could simply consist of recasting the problem as a set of independent binary quantification problems. Such a solution is simple but na\"ive, since the independence assumption upon which it rests is, in most cases, not satisfied. In these cases, knowing the relative frequency of one class could be of help in determining the prevalence of other related classes. We propose the first truly multi-label quantification methods, i.e., methods for inferring estimators of class prevalence values that strive to leverage the stochastic dependencies among the classes of interest in order to predict their relative frequencies more accurately. We show empirical evidence that natively multi-label solutions outperform the na\"ive approaches by a large margin. The code to reproduce all our experiments is available online.

==> tables/mlc_nocol.app.ae.tex <==

                \begin{tabular}{|l|c|ccccccc|} \cline{2-9}
\multicolumn{1}{c|}{} & \side{\bqbc} & \side{\textsc{ML-knn}\phantom{0}} & \side{\textsc{DT}} & \side{\textsc{RF}} & \side{\textsc{CChain}} & \side{\textsc{CLEMS}} & \side{\textsc{LSC}} & \side{\textsc{SG}} \\\hline
\texttt{Emotions} & .0569 \cellcolor{green!34} & .2292 \cellcolor{red!19} & .0772 \cellcolor{green!28} & .0575 \cellcolor{green!34} & .0626 \cellcolor{green!32} & .2292 \cellcolor{red!19} & .2785 \cellcolor{red!35} & \textbf{.0552} \cellcolor{green!35} \\\texttt{Scene} & .1046 \cellcolor{green!6} & .1541 \cellcolor{red!23} & .0686 \cellcolor{green!29} & .0691 \cellcolor{green!28} & \textbf{.0593} \cellcolor{green!35} & .1541 \cellcolor{red!23} & .1720 \cellcolor{red!35} & .0670 \cellcolor{green!30} \\\texttt{Yeast} & .1843 \cellcolor{red!8} & .1796 \cellcolor{red!6} & .0805 \cellcolor{green!31} & .0729 \cellcolor{green!34} & .0796 \cellcolor{green!32} & .1757 \cellcolor{red!5} & .2531 \cellcolor{red!35} & \textbf{.0722} \cellcolor{green!35} \\\texttt{Birds} & .0314 \cellcolor{green!8} & .0508 \cellcolor{red!33} & .0254 \cellcolor{green!20} & \textbf{.0187} \cellcolor{green!35} & .0227 \cellcolor{green!26} & .0508 \cellcolor{red!33} & .0517 \cellcolor{red!35} & .0232 \cellcolor{green!25} \\\texttt{Genbase} & .0011 \cellcolor{green!34} & .0570 \cellcolor{red!33} & .0011 \cellcolor{green!34} & .0036 \cellcolor{green!31} & .0006 \cellcolor{green!34} & .0570 \cellcolor{red!33} & .0583 \cellcolor{red!35} & \textbf{.0005} \cellcolor{green!35} \\\texttt{Medical} & \textbf{.0136} \cellcolor{green!35} & .0560 \cellcolor{red!27} & .0143 \cellcolor{green!33} & .0194 \cellcolor{green!26} & .0140 \cellcolor{green!34} & .0556 \cellcolor{red!27} & .0607 \cellcolor{red!35} & .0147 \cellcolor{green!33} \\\texttt{tmc2007\_500} & .1114 \cellcolor{red!35} & .0864 \cellcolor{red!19} & \textbf{.0013} \cellcolor{green!35} & .0133 \cellcolor{green!27} & .0262 \cellcolor{green!19} & .0867 \cellcolor{red!19} & .1035 \cellcolor{red!29} & .0264 \cellcolor{green!19} \\\texttt{Ohsumed} & .1059 \cellcolor{red!35} & .0728 \cellcolor{red!7} & .0318 \cellcolor{green!26} & .0304 \cellcolor{green!27} & \textbf{.0217} \cellcolor{green!35} & .0730 \cellcolor{red!7} & .0775 \cellcolor{red!11} & .0229 \cellcolor{green!34} \\\texttt{Enron} & .0364 \cellcolor{green!9} & .0584 \cellcolor{red!22} & .0231 \cellcolor{green!28} & .0195 \cellcolor{green!33} & .0188 \cellcolor{green!34} & .0588 \cellcolor{red!23} & .0670 \cellcolor{red!35} & \textbf{.0185} \cellcolor{green!35} \\\texttt{Reuters-21578} & .0184 \cellcolor{red!35} & .0173 \cellcolor{red!29} & .0064 \cellcolor{green!23} & .0081 \cellcolor{green!15} & .0041 \cellcolor{green!34} & .0174 \cellcolor{red!29} & .0180 \cellcolor{red!33} & \textbf{.0041} \cellcolor{green!35} \\\texttt{RCV1-v2} & .0492 \cellcolor{red!35} & .0332 \cellcolor{red!5} & .0175 \cellcolor{green!22} & .0200 \cellcolor{green!17} & .0112 \cellcolor{green!33} & .0332 \cellcolor{red!6} & .0358 \cellcolor{red!10} & \textbf{.0105} \cellcolor{green!35} \\\texttt{Mediamill} & .1713 \cellcolor{red!35} & .0367 \cellcolor{green!27} & .0227 \cellcolor{green!33} & .0214 \cellcolor{green!34} & .0244 \cellcolor{green!33} & .0394 \cellcolor{green!26} & .0438 \cellcolor{green!24} & \textbf{.0203} \cellcolor{green!35} \\\texttt{Bibtex} & .0358 \cellcolor{red!35} & .0167 \cellcolor{green!16} & .0113 \cellcolor{green!30} & .0098 \cellcolor{green!34} & .0099 \cellcolor{green!34} & .0168 \cellcolor{green!15} & .0168 \cellcolor{green!15} & \textbf{.0097} \cellcolor{green!35} \\\texttt{Corel5k} & .0582 \cellcolor{red!35} & .0109 \cellcolor{green!30} & .0133 \cellcolor{green!27} & .0080 \cellcolor{green!34} & .0088 \cellcolor{green!33} & .0111 \cellcolor{green!30} & .0110 \cellcolor{green!30} & \textbf{.0078} \cellcolor{green!35} \\\texttt{Delicious} & .1418 \cellcolor{red!35} & .0164 \cellcolor{green!31} & .0106 \cellcolor{green!34} & .0095 \cellcolor{green!34} & .0112 \cellcolor{green!33} & .0178 \cellcolor{green!30} & .0176 \cellcolor{green!30} & \textbf{.0092} \cellcolor{green!35} \\\hline
\multicolumn{1}{|c|}{Average} & .0725 \cellcolor{red!24} & .0696 \cellcolor{red!20} & .0264 \cellcolor{green!31} & .0251 \cellcolor{green!32} & .0242 \cellcolor{green!34} & .0697 \cellcolor{red!20} & .0815 \cellcolor{red!35} & \textbf{.0234} \cellcolor{green!35} \\\multicolumn{1}{|c|}{Rank Average} &  6.1 \cellcolor{red!21} &  5.5 \cellcolor{red!13} &  3.7 \cellcolor{green!9} &  2.9 \cellcolor{green!18} &  2.5 \cellcolor{green!24} &  6.3 \cellcolor{red!24} &  7.2 \cellcolor{red!35} & \textbf{1.7} \cellcolor{green!35} \\\hline

                \hline
                \end{tabular}
            

==> tables/mlq_nocol.app.ae.tex <==

                \begin{tabular}{|l|c|ccc|} \cline{2-5}
\multicolumn{1}{c|}{} & \side{\bqbc} & \side{\textsc{RakEL-Q}} & \side{\textsc{kMeans-Q}} & \side{\textsc{Reg-Q}} \\\hline
\texttt{Emotions} & .0569 \cellcolor{green!25} & .0589$^{\phantom{\ddag}}$ \cellcolor{green!13} & \textbf{.0552} \cellcolor{green!35} & .0674 \cellcolor{red!35} \\\texttt{Scene} & .1046 \cellcolor{red!35} & .0560$^{\phantom{\ddag}}$ \cellcolor{green!20} & .0603 \cellcolor{green!15} & \textbf{.0429} \cellcolor{green!35} \\\texttt{Yeast} & .1843 \cellcolor{red!35} & .0713$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0712 \cellcolor{green!34} & \textbf{.0701} \cellcolor{green!35} \\\texttt{Birds} & .0314 \cellcolor{red!35} & .0271$^{\phantom{\ddag}}$ \cellcolor{red!3} & .0221 \cellcolor{green!33} & \textbf{.0219} \cellcolor{green!35} \\\texttt{Genbase} & .0011 \cellcolor{green!12} & \textbf{.0005}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0014 \cellcolor{red!1} & .0023 \cellcolor{red!35} \\\texttt{Medical} & .0136 \cellcolor{green!34} & \textbf{.0135}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0136 \cellcolor{green!34} & .0230 \cellcolor{red!35} \\\texttt{tmc2007\_500} & .1114 \cellcolor{red!35} & .0255$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{.0244} \cellcolor{green!35} & .0252 \cellcolor{green!34} \\\texttt{Ohsumed} & .1059 \cellcolor{red!35} & .0218$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0221 \cellcolor{green!33} & \textbf{.0197} \cellcolor{green!35} \\\texttt{Enron} & .0364 \cellcolor{red!35} & .0189$^{\ddag}$ \cellcolor{green!34} & .0188 \cellcolor{green!34} & \textbf{.0187} \cellcolor{green!35} \\\texttt{Reuters-21578} & .0184 \cellcolor{red!35} & .0042$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{.0042} \cellcolor{green!35} & .0054 \cellcolor{green!29} \\\texttt{RCV1-v2} & .0492 \cellcolor{red!35} & \textbf{.0106}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0110 \cellcolor{green!34} & .0117 \cellcolor{green!32} \\\texttt{Mediamill} & .1713 \cellcolor{red!35} & .0210$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0211 \cellcolor{green!34} & \textbf{.0192} \cellcolor{green!35} \\\texttt{Bibtex} & .0358 \cellcolor{red!35} & .0097$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0097 \cellcolor{green!34} & \textbf{.0096} \cellcolor{green!35} \\\texttt{Corel5k} & .0582 \cellcolor{red!35} & .0080$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0081 \cellcolor{green!34} & \textbf{.0077} \cellcolor{green!35} \\\texttt{Delicious} & .1418 \cellcolor{red!35} & \textbf{.0094}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0096 \cellcolor{green!34} & .0095 \cellcolor{green!34} \\\hline
\multicolumn{1}{|c|}{Average} & .0725 \cellcolor{red!35} & .0231 \cellcolor{green!34} & \textbf{.0228} \cellcolor{green!35} & .0229 \cellcolor{green!34} \\\multicolumn{1}{|c|}{Rank Average} &  3.7 \cellcolor{red!35} &  2.1 \cellcolor{green!32} &  2.3 \cellcolor{green!23} & \textbf{2.0} \cellcolor{green!35} \\\hline

                \hline
                \end{tabular}
            

==> tables/mlq_nocol.drift.app.ae.tex <==

                \resizebox{\textwidth}{!}{% 
                    \begin{tabular}{|l|c|ccc|c|ccc|c|ccc|} \cline{2-13}
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{low shift} & \multicolumn{4}{c|}{mid shift} & \multicolumn{4}{c|}{high shift}\\\cline{2-13}

\multicolumn{1}{c|}{} & \side{\bqbc} & \side{\textsc{RakEL-Q}} & \side{\textsc{kMeans-Q}} & \side{\textsc{Reg-Q}} & \side{\bqbc} & \side{\textsc{RakEL-Q}} & \side{\textsc{kMeans-Q}} & \side{\textsc{Reg-Q}} & \side{\bqbc} & \side{\textsc{RakEL-Q}} & \side{\textsc{kMeans-Q}} & \side{\textsc{Reg-Q}}\\\hline
\texttt{Emotions} & .0418$^{\ddag}$ \cellcolor{green!34} & .0451$^{\phantom{\ddag}}$ \cellcolor{green!20} & \textbf{.0416} \cellcolor{green!35} & .0586 \cellcolor{red!35} & .0685 \cellcolor{green!4} & .0687 \cellcolor{green!1} & \textbf{.0657} \cellcolor{green!35} & .0720 \cellcolor{red!35} & .0923 \cellcolor{red!11} & .0940$^{\phantom{\ddag}}$ \cellcolor{red!25} & \textbf{.0869} \cellcolor{green!35} & .0951 \cellcolor{red!35} \\
\texttt{Scene} & .0842$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.0333}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0345 \cellcolor{green!33} & .0384 \cellcolor{green!27} & .1140 \cellcolor{red!35} & .0680 \cellcolor{green!12} & .0735 \cellcolor{green!6} & \textbf{.0459} \cellcolor{green!35} & .1427 \cellcolor{red!35} & .0961$^{\phantom{\ddag}}$ \cellcolor{green!0} & .1063 \cellcolor{red!7} & \textbf{.0499} \cellcolor{green!35} \\
\texttt{Yeast} & .1756$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0443$^{\ddag}$ \cellcolor{green!34} & \textbf{.0443} \cellcolor{green!35} & .0480 \cellcolor{green!33} & .1900 \cellcolor{red!35} & .0972 \cellcolor{green!30} & .0970 \cellcolor{green!30} & \textbf{.0913} \cellcolor{green!35} & .2206 \cellcolor{red!35} & .1520$^{\phantom{\ddag}}$ \cellcolor{green!21} & .1521 \cellcolor{green!21} & \textbf{.1361} \cellcolor{green!35} \\
\texttt{Birds} & .0286$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0242$^{\phantom{\ddag}}$ \cellcolor{red!5} & .0194 \cellcolor{green!26} & \textbf{.0181} \cellcolor{green!35} & .0328 \cellcolor{red!35} & .0286 \cellcolor{red!2} & \textbf{.0237} \cellcolor{green!35} & .0243 \cellcolor{green!30} & .0440 \cellcolor{red!35} & .0405$^{\phantom{\ddag}}$ \cellcolor{red!15} & \textbf{.0317} \cellcolor{green!35} & .0351 \cellcolor{green!15} \\
\texttt{Genbase} & .0011$^{\phantom{\ddag}}$ \cellcolor{green!10} & \textbf{.0005}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0014 \cellcolor{red!2} & .0022 \cellcolor{red!35} & .0011 \cellcolor{green!14} & \textbf{.0005} \cellcolor{green!35} & .0015 \cellcolor{green!0} & .0025 \cellcolor{red!35} & .0010 \cellcolor{green!11} & \textbf{.0004}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0013 \cellcolor{green!0} & .0023 \cellcolor{red!35} \\
\texttt{Medical} & .0127$^{\phantom{\ddag}}$ \cellcolor{green!29} & \textbf{.0122}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0130 \cellcolor{green!26} & .0191 \cellcolor{red!35} & .0146 \cellcolor{green!32} & .0149 \cellcolor{green!31} & \textbf{.0142} \cellcolor{green!35} & .0279 \cellcolor{red!35} & .0169 \cellcolor{green!31} & .0181$^{\phantom{\ddag}}$ \cellcolor{green!26} & \textbf{.0158} \cellcolor{green!35} & .0351 \cellcolor{red!35} \\
\texttt{tmc2007\_500} & .1108$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0188$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{.0182} \cellcolor{green!35} & .0213 \cellcolor{green!32} & .1154 \cellcolor{red!35} & .0319 \cellcolor{green!32} & .0303 \cellcolor{green!34} & \textbf{.0292} \cellcolor{green!35} & .1008 \cellcolor{red!35} & .0385$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0354 \cellcolor{green!31} & \textbf{.0321} \cellcolor{green!35} \\
\texttt{Ohsumed} & .1004$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.0171}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0174 \cellcolor{green!34} & .0183 \cellcolor{green!34} & .1087 \cellcolor{red!35} & .0249 \cellcolor{green!31} & .0251 \cellcolor{green!31} & \textbf{.0209} \cellcolor{green!35} & .1177 \cellcolor{red!35} & .0300$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0304 \cellcolor{green!28} & \textbf{.0215} \cellcolor{green!35} \\
\texttt{Enron} & .0347$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0163$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{.0163} \cellcolor{green!35} & .0169 \cellcolor{green!32} & .0397 \cellcolor{red!35} & .0242 \cellcolor{green!28} & .0239 \cellcolor{green!29} & \textbf{.0227} \cellcolor{green!35} & .0439 \cellcolor{red!35} & .0301$^{\phantom{\ddag}}$ \cellcolor{green!16} & .0297 \cellcolor{green!18} & \textbf{.0253} \cellcolor{green!35} \\
\texttt{Reuters-21578} & .0167$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.0037}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0037 \cellcolor{green!34} & .0049 \cellcolor{green!28} & .0243 \cellcolor{red!35} & .0062 \cellcolor{green!34} & \textbf{.0060} \cellcolor{green!35} & .0070 \cellcolor{green!31} & .0370 \cellcolor{red!35} & .0081$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{.0077} \cellcolor{green!35} & .0088 \cellcolor{green!32} \\
\texttt{RCV1-v2} & .0456$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.0085}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0089 \cellcolor{green!34} & .0093 \cellcolor{green!33} & .0533 \cellcolor{red!35} & \textbf{.0130} \cellcolor{green!35} & .0135 \cellcolor{green!34} & .0146 \cellcolor{green!32} & .0654 \cellcolor{red!35} & \textbf{.0196}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0205 \cellcolor{green!33} & .0215 \cellcolor{green!32} \\
\texttt{Mediamill} & .1697$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0159$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0159 \cellcolor{green!34} & \textbf{.0157} \cellcolor{green!35} & .1736 \cellcolor{red!35} & .0297 \cellcolor{green!32} & .0298 \cellcolor{green!32} & \textbf{.0251} \cellcolor{green!35} & .1806 \cellcolor{red!35} & .0413$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0414 \cellcolor{green!30} & \textbf{.0322} \cellcolor{green!35} \\
\texttt{Bibtex} & .0354$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0092$^{\dag\phantom{\dag}}$ \cellcolor{green!34} & \textbf{.0092} \cellcolor{green!35} & .0092 \cellcolor{green!34} & .0374 \cellcolor{red!35} & .0126 \cellcolor{green!32} & .0127 \cellcolor{green!32} & \textbf{.0116} \cellcolor{green!35} & .0423 \cellcolor{red!35} & .0153$^{\phantom{\ddag}}$ \cellcolor{green!29} & .0154 \cellcolor{green!28} & \textbf{.0129} \cellcolor{green!35} \\
\texttt{Corel5k} & .0582$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0079$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0080 \cellcolor{green!34} & \textbf{.0075} \cellcolor{green!35} & .0585 \cellcolor{red!35} & .0086 \cellcolor{green!34} & .0088 \cellcolor{green!34} & \textbf{.0082} \cellcolor{green!35} & .0594 \cellcolor{red!35} & .0088$^{\dag\phantom{\dag}}$ \cellcolor{green!34} & .0096 \cellcolor{green!33} & \textbf{.0087} \cellcolor{green!35} \\
\texttt{Delicious} & .1420$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.0089}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0091 \cellcolor{green!34} & .0093 \cellcolor{green!34} & .1417 \cellcolor{red!35} & .0121 \cellcolor{green!34} & .0124 \cellcolor{green!34} & \textbf{.0109} \cellcolor{green!35} & .1238 \cellcolor{red!35} & .0126$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0131 \cellcolor{green!33} & \textbf{.0104} \cellcolor{green!35} \\
\hline
\multicolumn{1}{|c|}{Average} & .0677 \cellcolor{red!35} & .0159 \cellcolor{green!34} & \textbf{.0157} \cellcolor{green!35} & .0177 \cellcolor{green!32} & .0761 \cellcolor{red!35} & .0308 \cellcolor{green!32} & .0303 \cellcolor{green!32} & \textbf{.0288} \cellcolor{green!35} & .1012 \cellcolor{red!35} & .0560 \cellcolor{green!21} & .0564 \cellcolor{green!20} & \textbf{.0452} \cellcolor{green!35} \\
\multicolumn{1}{|c|}{Rank Average} &  3.6 \cellcolor{red!35} & \textbf{1.7} \cellcolor{green!35} &  1.9 \cellcolor{green!25} &  2.8 \cellcolor{red!6} &  3.6 \cellcolor{red!35} &  2.3 \cellcolor{green!21} &  2.2 \cellcolor{green!23} & \textbf{1.9} \cellcolor{green!35} &  3.6 \cellcolor{red!35} &  2.2 \cellcolor{green!23} &  2.3 \cellcolor{green!21} & \textbf{1.9} \cellcolor{green!35} \\

                \hline
                \end{tabular}%
                }
            

==> tables/mlq_nocol.drift.app.mrae.tex <==

                \resizebox{\textwidth}{!}{% 
                    \begin{tabular}{|l|c|ccc|c|ccc|c|ccc|} \cline{2-13}
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{low shift} & \multicolumn{4}{c|}{mid shift} & \multicolumn{4}{c|}{high shift}\\\cline{2-13}

\multicolumn{1}{c|}{} & \side{\bqbc} & \side{\textsc{RakEL-Q}} & \side{\textsc{kMeans-Q}} & \side{\textsc{Reg-Q}} & \side{\bqbc} & \side{\textsc{RakEL-Q}} & \side{\textsc{kMeans-Q}} & \side{\textsc{Reg-Q}} & \side{\bqbc} & \side{\textsc{RakEL-Q}} & \side{\textsc{kMeans-Q}} & \side{\textsc{Reg-Q}}\\\hline
\texttt{Emotions} & .1045 \cellcolor{green!32} & .1119 \cellcolor{green!20} & \textbf{.1028} \cellcolor{green!35} & .1454 \cellcolor{red!35} & .3657$^{\ddag}$ \cellcolor{red!35} & .3507$^{\ddag}$ \cellcolor{red!20} & .3490 \cellcolor{red!18} & \textbf{.2935} \cellcolor{green!35} & .5430 \cellcolor{red!15} & .5707 \cellcolor{red!35} & .5265$^{\phantom{\ddag}}$ \cellcolor{red!3} & \textbf{.4726} \cellcolor{green!35} \\
\texttt{Scene} & .4068 \cellcolor{red!35} & .1540 \cellcolor{green!34} & .1612 \cellcolor{green!32} & \textbf{.1519} \cellcolor{green!35} & .7417$^{\phantom{\ddag}}$ \cellcolor{red!35} & .3454$^{\phantom{\ddag}}$ \cellcolor{green!21} & .3696 \cellcolor{green!18} & \textbf{.2515} \cellcolor{green!35} &  3.4909 \cellcolor{red!35} &  2.1628 \cellcolor{green!3} &  2.3644$^{\phantom{\ddag}}$ \cellcolor{red!2} & \textbf{1.0550} \cellcolor{green!35} \\
\texttt{Yeast} & .9286 \cellcolor{red!35} & \textbf{.2037} \cellcolor{green!35} & .2049 \cellcolor{green!34} & .2084 \cellcolor{green!34} &  1.0377$^{\phantom{\ddag}}$ \cellcolor{red!35} & .4173$^{\phantom{\ddag}}$ \cellcolor{green!31} & .4187 \cellcolor{green!31} & \textbf{.3816} \cellcolor{green!35} &  1.6070 \cellcolor{red!35} &  1.1721 \cellcolor{green!20} &  1.1786$^{\phantom{\ddag}}$ \cellcolor{green!19} & \textbf{1.0586} \cellcolor{green!35} \\
\texttt{Birds} & .5500 \cellcolor{red!35} & .3923 \cellcolor{green!3} & .3263 \cellcolor{green!19} & \textbf{.2646} \cellcolor{green!35} & .6844$^{\phantom{\ddag}}$ \cellcolor{red!35} & .4967$^{\phantom{\ddag}}$ \cellcolor{green!2} & .4161 \cellcolor{green!19} & \textbf{.3372} \cellcolor{green!35} &  1.0065 \cellcolor{red!35} & .6907 \cellcolor{red!0} & .5887$^{\phantom{\ddag}}$ \cellcolor{green!10} & \textbf{.3643} \cellcolor{green!35} \\
\texttt{Genbase} & .0472 \cellcolor{green!4} & \textbf{.0155} \cellcolor{green!35} & .0351 \cellcolor{green!15} & .0874 \cellcolor{red!35} & .0506$^{\phantom{\ddag}}$ \cellcolor{green!4} & \textbf{.0166}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0362 \cellcolor{green!17} & .0947 \cellcolor{red!35} & .0530 \cellcolor{red!1} & \textbf{.0161} \cellcolor{green!35} & .0358$^{\phantom{\ddag}}$ \cellcolor{green!15} & .0864 \cellcolor{red!35} \\
\texttt{Medical} & .1725 \cellcolor{green!26} & .1879 \cellcolor{green!21} & \textbf{.1487} \cellcolor{green!35} & .3463 \cellcolor{red!35} & .2177$^{\phantom{\ddag}}$ \cellcolor{green!27} & .2553$^{\phantom{\ddag}}$ \cellcolor{green!19} & \textbf{.1803} \cellcolor{green!35} & .5229 \cellcolor{red!35} & .3974 \cellcolor{green!26} & .4843 \cellcolor{green!16} & \textbf{.3328}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .8961 \cellcolor{red!35} \\
\texttt{tmc2007\_500} &  1.9392 \cellcolor{red!35} & .1892 \cellcolor{green!34} & \textbf{.1735} \cellcolor{green!35} & .2626 \cellcolor{green!31} &  2.1917$^{\phantom{\ddag}}$ \cellcolor{red!35} & .2964$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{.2709} \cellcolor{green!35} & .3226 \cellcolor{green!33} &  2.4020 \cellcolor{red!35} & .5277 \cellcolor{green!32} & .4822$^{\dag\phantom{\dag}}$ \cellcolor{green!34} & \textbf{.4660} \cellcolor{green!35} \\
\texttt{Ohsumed} &  1.9122 \cellcolor{red!35} & \textbf{.1687} \cellcolor{green!35} & .1876 \cellcolor{green!34} & .2285 \cellcolor{green!32} &  2.3257$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.2275}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .2519 \cellcolor{green!34} & .2736 \cellcolor{green!33} &  2.9609 \cellcolor{red!35} & .4925 \cellcolor{green!32} & .5201$^{\phantom{\ddag}}$ \cellcolor{green!31} & \textbf{.3872} \cellcolor{green!35} \\
\texttt{Enron} & .6213 \cellcolor{red!35} & \textbf{.2876} \cellcolor{green!35} & .3000 \cellcolor{green!32} & .3272 \cellcolor{green!26} & .7415$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.3847}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .3972 \cellcolor{green!32} & .4117 \cellcolor{green!29} &  1.1457 \cellcolor{red!35} & .6518 \cellcolor{green!24} & .6627$^{\phantom{\ddag}}$ \cellcolor{green!23} & \textbf{.5685} \cellcolor{green!35} \\
\texttt{Reuters-21578} & .9101 \cellcolor{red!35} & \textbf{.0890} \cellcolor{green!35} & .0936 \cellcolor{green!34} & .1389 \cellcolor{green!30} &  1.1838$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.1091}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .1125 \cellcolor{green!34} & .1740 \cellcolor{green!30} &  1.0398 \cellcolor{red!35} & \textbf{.1091} \cellcolor{green!35} & .1145$^{\phantom{\ddag}}$ \cellcolor{green!34} & .1616 \cellcolor{green!31} \\
\texttt{RCV1-v2} &  2.0283 \cellcolor{red!35} & \textbf{.1480} \cellcolor{green!35} & .2005 \cellcolor{green!33} & .1896 \cellcolor{green!33} &  2.5246$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.2026}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .2687 \cellcolor{green!33} & .2836 \cellcolor{green!32} &  2.9699 \cellcolor{red!35} & \textbf{.3350} \cellcolor{green!35} & .4316$^{\phantom{\ddag}}$ \cellcolor{green!32} & .5063 \cellcolor{green!30} \\
\texttt{Mediamill} &  7.6767 \cellcolor{red!35} & .3203 \cellcolor{green!34} & .3214 \cellcolor{green!34} & \textbf{.2708} \cellcolor{green!35} &  8.6165$^{\phantom{\ddag}}$ \cellcolor{red!35} & .4931$^{\phantom{\ddag}}$ \cellcolor{green!33} & .4933 \cellcolor{green!33} & \textbf{.3722} \cellcolor{green!35} &  8.9409 \cellcolor{red!35} & .7837 \cellcolor{green!32} & .7821$^{\phantom{\ddag}}$ \cellcolor{green!32} & \textbf{.5320} \cellcolor{green!35} \\
\texttt{Bibtex} &  1.6686 \cellcolor{red!35} & \textbf{.3097} \cellcolor{green!35} & .3183 \cellcolor{green!34} & .3532 \cellcolor{green!32} &  1.6432$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.3180}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .3320 \cellcolor{green!34} & .3297 \cellcolor{green!34} &  1.5127 \cellcolor{red!35} & .3186 \cellcolor{green!34} & .3338$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{.3046} \cellcolor{green!35} \\
\texttt{Corel5k} &  2.2844 \cellcolor{red!35} & \textbf{.2205} \cellcolor{green!35} & .2941 \cellcolor{green!32} & .2299 \cellcolor{green!34} &  2.5112$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.2337}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .3164 \cellcolor{green!32} & .2458 \cellcolor{green!34} &  2.9733 \cellcolor{red!35} & \textbf{.2669} \cellcolor{green!35} & .3760$^{\phantom{\ddag}}$ \cellcolor{green!32} & .2898 \cellcolor{green!34} \\
\texttt{Delicious} &  6.6314 \cellcolor{red!35} & .3309 \cellcolor{green!34} & .3353 \cellcolor{green!34} & \textbf{.3012} \cellcolor{green!35} &  7.4738$^{\phantom{\ddag}}$ \cellcolor{red!35} & .4034$^{\phantom{\ddag}}$ \cellcolor{green!34} & .4165 \cellcolor{green!34} & \textbf{.3357} \cellcolor{green!35} &  7.3272 \cellcolor{red!35} & .4569 \cellcolor{green!34} & .4822$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{.3599} \cellcolor{green!35} \\
\hline
\multicolumn{1}{|c|}{Average} &  1.9897 \cellcolor{red!35} & \textbf{.2101} \cellcolor{green!35} & .2188 \cellcolor{green!34} & .2366 \cellcolor{green!33} &  1.9312 \cellcolor{red!35} & \textbf{.3035} \cellcolor{green!35} & .3058 \cellcolor{green!34} & .3043 \cellcolor{green!34} &  2.4206 \cellcolor{red!35} & .8541 \cellcolor{green!26} & .8796 \cellcolor{green!25} & \textbf{.6270} \cellcolor{green!35} \\
\multicolumn{1}{|c|}{Rank Average} &  3.7 \cellcolor{red!35} & \textbf{1.7} \cellcolor{green!35} &  2.1 \cellcolor{green!18} &  2.5 \cellcolor{green!4} &  3.8 \cellcolor{red!35} & \textbf{1.7} \cellcolor{green!35} &  2.3 \cellcolor{green!16} &  2.2 \cellcolor{green!19} &  3.7 \cellcolor{red!35} &  2.1 \cellcolor{green!21} &  2.4 \cellcolor{green!11} & \textbf{1.7} \cellcolor{green!35} \\

                \hline
                \end{tabular}%
                }
            

==> tables/mlqreg_col.app.ae.tex <==

            \resizebox{\textwidth}{!}{%
                    \begin{tabular}{|l|cccccc|cccccc|cccccc|} \cline{2-19}
\multicolumn{1}{c|}{} & \multicolumn{6}{c|}{low shift} & \multicolumn{6}{c|}{mid shift} & \multicolumn{6}{c|}{high shift}\\\cline{2-19}

\multicolumn{1}{c|}{} & \side{R1} & \side{R2} & \side{R3} & MRQ-PCC & \side{R5} & \side{R6} & \side{R1} & \side{R2} & \side{R3} & MRQ-PCC & \side{R5} & \side{R6} & \side{R1} & \side{R2} & \side{R3} & MRQ-PCC & \side{R5} & \side{R6}\\\hline
\texttt{Emotions} & .050 \cellcolor{green!29} & .063 \cellcolor{red!16} & \textbf{.048} \cellcolor{green!35} & .059 \cellcolor{red!0} & .069 \cellcolor{red!35} & .057 \cellcolor{green!3} & \textbf{.063} \cellcolor{green!35} & .081 \cellcolor{green!10} & .071 \cellcolor{green!24} & .072 \cellcolor{green!22} & .104 \cellcolor{red!19} & .115 \cellcolor{red!35} & \textbf{.078} \cellcolor{green!35} & .103 \cellcolor{green!17} & .124$^{\phantom{\ddag}}$ \cellcolor{green!2} & .095 \cellcolor{green!22} & .130 \cellcolor{red!1} & .177 \cellcolor{red!35} \\
\texttt{Scene} & .035 \cellcolor{green!11} & .044 \cellcolor{red!35} & \textbf{.030} \cellcolor{green!35} & .038 \cellcolor{red!6} & .036 \cellcolor{green!4} & .036 \cellcolor{green!6} & .045 \cellcolor{green!22} & .111 \cellcolor{red!35} & \textbf{.031} \cellcolor{green!35} & .046 \cellcolor{green!21} & .086 \cellcolor{red!13} & .087 \cellcolor{red!13} & .058 \cellcolor{green!30} & .176 \cellcolor{red!35} & .051$^{\dag\phantom{\dag}}$ \cellcolor{green!34} & \textbf{.050} \cellcolor{green!35} & .125 \cellcolor{red!6} & .126 \cellcolor{red!7} \\
\texttt{Yeast} & .048 \cellcolor{green!21} & .049 \cellcolor{green!12} & .056 \cellcolor{red!35} & .048 \cellcolor{green!19} & \textbf{.046} \cellcolor{green!35} & .046 \cellcolor{green!29} & .092 \cellcolor{green!29} & .094 \cellcolor{green!12} & .096 \cellcolor{green!1} & \textbf{.091} \cellcolor{green!35} & .098 \cellcolor{red!18} & .100 \cellcolor{red!35} & .137 \cellcolor{green!30} & .142 \cellcolor{green!10} & .152$^{\phantom{\ddag}}$ \cellcolor{red!25} & \textbf{.136} \cellcolor{green!35} & .152 \cellcolor{red!25} & .154 \cellcolor{red!35} \\
\texttt{Birds} & .021 \cellcolor{red!10} & .023 \cellcolor{red!35} & .018 \cellcolor{green!29} & \textbf{.018} \cellcolor{green!35} & .022 \cellcolor{red!16} & .021 \cellcolor{red!10} & .029 \cellcolor{red!22} & .030 \cellcolor{red!35} & .025 \cellcolor{green!24} & \textbf{.024} \cellcolor{green!35} & .030 \cellcolor{red!32} & .028 \cellcolor{red!10} & .040 \cellcolor{red!9} & .042 \cellcolor{red!24} & .038$^{\phantom{\ddag}}$ \cellcolor{green!9} & \textbf{.035} \cellcolor{green!35} & .044 \cellcolor{red!35} & .043 \cellcolor{red!27} \\
\texttt{Genbase} & \textbf{.001} \cellcolor{green!35} & .014 \cellcolor{red!17} & .010 \cellcolor{red!3} & .002 \cellcolor{green!31} & .017 \cellcolor{red!30} & .018 \cellcolor{red!35} & \textbf{.001} \cellcolor{green!35} & .018 \cellcolor{red!13} & .015 \cellcolor{red!5} & .002 \cellcolor{green!31} & .025 \cellcolor{red!34} & .025 \cellcolor{red!35} & \textbf{.001} \cellcolor{green!35} & .017 \cellcolor{green!3} & .017$^{\phantom{\ddag}}$ \cellcolor{green!3} & .002 \cellcolor{green!33} & .036 \cellcolor{red!35} & .035 \cellcolor{red!31} \\
\texttt{Medical} & .023 \cellcolor{red!35} & \textbf{.019} \cellcolor{green!35} & .020 \cellcolor{green!9} & .019 \cellcolor{green!26} & .021 \cellcolor{green!0} & .019 \cellcolor{green!21} & .031 \cellcolor{green!11} & \textbf{.026} \cellcolor{green!35} & .039 \cellcolor{red!35} & .028 \cellcolor{green!26} & .032 \cellcolor{green!6} & .027 \cellcolor{green!33} & .036 \cellcolor{green!24} & \textbf{.031} \cellcolor{green!35} & .065$^{\phantom{\ddag}}$ \cellcolor{red!35} & .035 \cellcolor{green!27} & .044 \cellcolor{green!9} & .038 \cellcolor{green!21} \\
\texttt{tmc2007\_500} & .023 \cellcolor{green!24} & .026 \cellcolor{green!1} & \textbf{.021} \cellcolor{green!35} & .021 \cellcolor{green!34} & .031 \cellcolor{red!35} & .027 \cellcolor{red!7} & .027 \cellcolor{green!23} & .044 \cellcolor{red!13} & \textbf{.022} \cellcolor{green!35} & .029 \cellcolor{green!19} & .053 \cellcolor{red!35} & .051 \cellcolor{red!30} & .028 \cellcolor{green!28} & .057 \cellcolor{red!12} & \textbf{.024}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .032 \cellcolor{green!23} & .073 \cellcolor{red!35} & .071 \cellcolor{red!33} \\
\texttt{Ohsumed} & .019 \cellcolor{green!20} & .022 \cellcolor{red!18} & .018 \cellcolor{green!34} & \textbf{.018} \cellcolor{green!35} & .023 \cellcolor{red!35} & .023 \cellcolor{red!33} & .021 \cellcolor{green!28} & .036 \cellcolor{red!15} & \textbf{.018} \cellcolor{green!35} & .021 \cellcolor{green!28} & .043 \cellcolor{red!35} & .043 \cellcolor{red!33} & .022 \cellcolor{green!31} & .047 \cellcolor{red!12} & \textbf{.020}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .022 \cellcolor{green!32} & .060 \cellcolor{red!35} & .059 \cellcolor{red!33} \\
\texttt{Enron} & .019 \cellcolor{red!35} & .019 \cellcolor{red!21} & .017 \cellcolor{green!19} & \textbf{.017} \cellcolor{green!35} & .018 \cellcolor{green!0} & .019 \cellcolor{red!26} & .025 \cellcolor{red!8} & .026 \cellcolor{red!17} & \textbf{.022} \cellcolor{green!35} & .023 \cellcolor{green!24} & .027 \cellcolor{red!31} & .027 \cellcolor{red!35} & .029 \cellcolor{red!8} & .030 \cellcolor{red!16} & \textbf{.021}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .025 \cellcolor{green!11} & .033 \cellcolor{red!35} & .032 \cellcolor{red!30} \\
\texttt{Reuters-21578} & \textbf{.005} \cellcolor{green!35} & .007 \cellcolor{red!14} & .007 \cellcolor{red!15} & .005 \cellcolor{green!31} & .008 \cellcolor{red!34} & .008 \cellcolor{red!35} & \textbf{.007} \cellcolor{green!35} & .011 \cellcolor{green!7} & .011 \cellcolor{green!10} & .007 \cellcolor{green!34} & .018 \cellcolor{red!34} & .018 \cellcolor{red!35} & .010 \cellcolor{green!29} & .014 \cellcolor{green!14} & .014$^{\phantom{\ddag}}$ \cellcolor{green!17} & \textbf{.009} \cellcolor{green!35} & .027 \cellcolor{red!30} & .028 \cellcolor{red!35} \\
\texttt{RCV1-v2} & .009 \cellcolor{green!33} & .013 \cellcolor{red!10} & .013 \cellcolor{red!6} & \textbf{.009} \cellcolor{green!35} & .015 \cellcolor{red!35} & .015 \cellcolor{red!34} & \textbf{.014} \cellcolor{green!35} & .025 \cellcolor{red!11} & .021 \cellcolor{green!5} & .015 \cellcolor{green!34} & .030 \cellcolor{red!34} & .030 \cellcolor{red!35} & .022 \cellcolor{green!33} & .037 \cellcolor{red!6} & .037$^{\phantom{\ddag}}$ \cellcolor{red!7} & \textbf{.021} \cellcolor{green!35} & .047 \cellcolor{red!35} & .047 \cellcolor{red!34} \\
\texttt{Mediamill} & .018 \cellcolor{red!35} & .017 \cellcolor{green!3} & .016 \cellcolor{green!32} & \textbf{.016} \cellcolor{green!35} & .017 \cellcolor{green!7} & .018 \cellcolor{red!14} & .026 \cellcolor{green!11} & .027 \cellcolor{green!6} & \textbf{.023} \cellcolor{green!35} & .025 \cellcolor{green!18} & .032 \cellcolor{red!30} & .032 \cellcolor{red!35} & .032 \cellcolor{green!24} & .032 \cellcolor{green!22} & \textbf{.029}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .032 \cellcolor{green!21} & .044 \cellcolor{red!33} & .044 \cellcolor{red!35} \\
\texttt{Bibtex} & .010 \cellcolor{green!15} & .010 \cellcolor{red!10} & .010 \cellcolor{red!9} & \textbf{.009} \cellcolor{green!35} & .011 \cellcolor{red!16} & .011 \cellcolor{red!35} & .013 \cellcolor{green!22} & .015 \cellcolor{red!16} & .015 \cellcolor{red!6} & \textbf{.012} \cellcolor{green!35} & .017 \cellcolor{red!35} & .016 \cellcolor{red!20} & .014 \cellcolor{green!27} & .020 \cellcolor{red!15} & .020$^{\phantom{\ddag}}$ \cellcolor{red!16} & \textbf{.013} \cellcolor{green!35} & .022 \cellcolor{red!35} & .020 \cellcolor{red!15} \\
\texttt{Corel5k} & .007 \cellcolor{green!30} & .008 \cellcolor{green!5} & .009 \cellcolor{red!21} & .008 \cellcolor{green!25} & \textbf{.007} \cellcolor{green!35} & .009 \cellcolor{red!35} & .008 \cellcolor{green!29} & .009 \cellcolor{green!15} & .009 \cellcolor{green!2} & \textbf{.008} \cellcolor{green!35} & .009 \cellcolor{green!15} & .010 \cellcolor{red!35} & .009 \cellcolor{green!20} & .010 \cellcolor{green!9} & .010$^{\phantom{\ddag}}$ \cellcolor{green!6} & \textbf{.009} \cellcolor{green!35} & .011 \cellcolor{red!8} & .012 \cellcolor{red!35} \\
\texttt{Delicious} & \textbf{.009} \cellcolor{green!35} & .010 \cellcolor{green!22} & .009 \cellcolor{green!32} & .009 \cellcolor{green!32} & .010 \cellcolor{green!1} & .011 \cellcolor{red!35} & .011 \cellcolor{green!25} & .013 \cellcolor{red!14} & \textbf{.010} \cellcolor{green!35} & .011 \cellcolor{green!24} & .014 \cellcolor{red!21} & .015 \cellcolor{red!35} & .010 \cellcolor{green!26} & .015 \cellcolor{red!16} & \textbf{.009}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .010 \cellcolor{green!25} & .016 \cellcolor{red!26} & .017 \cellcolor{red!35} \\
\hline
\multicolumn{1}{|c|}{Average} & .010 \cellcolor{green!25} & .011 \cellcolor{red!0} & .011 \cellcolor{green!9} & \textbf{.010} \cellcolor{green!35} & .012 \cellcolor{red!11} & .012 \cellcolor{red!35} & .016 \cellcolor{green!32} & .022 \cellcolor{red!9} & .018 \cellcolor{green!23} & \textbf{.016} \cellcolor{green!35} & .024 \cellcolor{red!32} & .025 \cellcolor{red!35} & .024 \cellcolor{green!33} & .035 \cellcolor{red!8} & .028 \cellcolor{green!18} & \textbf{.024} \cellcolor{green!35} & .041 \cellcolor{red!32} & .041 \cellcolor{red!35} \\
\multicolumn{1}{|c|}{Rank Average} &  2.9 \cellcolor{green!12} &  4.1 \cellcolor{red!21} &  2.8 \cellcolor{green!16} & \textbf{2.1} \cellcolor{green!35} &  4.4 \cellcolor{red!29} &  4.6 \cellcolor{red!35} & \textbf{2.1} \cellcolor{green!35} &  4.0 \cellcolor{red!6} &  2.5 \cellcolor{green!27} &  2.1 \cellcolor{green!35} &  5.0 \cellcolor{red!29} &  5.3 \cellcolor{red!35} &  2.2 \cellcolor{green!27} &  3.6 \cellcolor{red!0} &  2.9 \cellcolor{green!13} & \textbf{1.8} \cellcolor{green!35} &  5.3 \cellcolor{red!35} &  5.2 \cellcolor{red!32} \\

            \hline
            \end{tabular}%
            }
        

==> tables/mlqreg_nocol.app.ae.tex <==

                \begin{tabular}{|l|c|cccccc|} \cline{2-8}
\multicolumn{1}{c|}{} & \side{\bqbc} & \side{Ridge} & \side{MultitaskLasso} & \side{RandomForest} & \side{StackedLinearSVR} & \side{ChainedLinearSVR\phantom{0}} & \side{LinearSVR} \\\hline
\texttt{Emotions} & \textbf{.0569} \cellcolor{green!35} & .0576$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0740 \cellcolor{green!0} & .0646 \cellcolor{green!19} & .0880 \cellcolor{red!28} & .0912 \cellcolor{red!35} & .0674 \cellcolor{green!13} \\\texttt{Scene} & .1046 \cellcolor{red!35} & .0427$^{\phantom{\ddag}}$ \cellcolor{green!26} & .0901 \cellcolor{red!20} & \textbf{.0344} \cellcolor{green!35} & .0687 \cellcolor{green!0} & .0689 \cellcolor{green!0} & .0429 \cellcolor{green!26} \\\texttt{Yeast} & .1843 \cellcolor{red!35} & .0702$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0722 \cellcolor{green!33} & .0776 \cellcolor{green!30} & .0724 \cellcolor{green!33} & .0738 \cellcolor{green!32} & \textbf{.0701} \cellcolor{green!35} \\\texttt{Birds} & .0314 \cellcolor{red!35} & .0260$^{\phantom{\ddag}}$ \cellcolor{green!5} & .0274 \cellcolor{red!5} & .0227 \cellcolor{green!29} & .0267 \cellcolor{red!0} & .0256 \cellcolor{green!7} & \textbf{.0219} \cellcolor{green!35} \\\texttt{Genbase} & \textbf{.0011} \cellcolor{green!35} & .0014$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0154 \cellcolor{red!14} & .0124 \cellcolor{red!4} & .0207 \cellcolor{red!33} & .0212 \cellcolor{red!35} & .0023 \cellcolor{green!30} \\\texttt{Medical} & \textbf{.0136} \cellcolor{green!35} & .0263$^{\phantom{\ddag}}$ \cellcolor{red!20} & .0219 \cellcolor{red!1} & .0297 \cellcolor{red!35} & .0259 \cellcolor{red!18} & .0231 \cellcolor{red!6} & .0230 \cellcolor{red!5} \\\texttt{tmc2007\_500} & .1114 \cellcolor{red!35} & .0249$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0355 \cellcolor{green!24} & \textbf{.0219} \cellcolor{green!35} & .0432 \cellcolor{green!18} & .0403 \cellcolor{green!20} & .0252 \cellcolor{green!32} \\\texttt{Ohsumed} & .1059 \cellcolor{red!35} & .0202$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0308 \cellcolor{green!25} & \textbf{.0186} \cellcolor{green!35} & .0357 \cellcolor{green!21} & .0353 \cellcolor{green!21} & .0197 \cellcolor{green!34} \\\texttt{Enron} & .0364 \cellcolor{red!35} & .0211$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0210 \cellcolor{green!26} & \textbf{.0187} \cellcolor{green!35} & .0209 \cellcolor{green!26} & .0215 \cellcolor{green!23} & .0187 \cellcolor{green!34} \\\texttt{Reuters-21578} & .0184 \cellcolor{red!35} & \textbf{.0053}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0081 \cellcolor{green!20} & .0080 \cellcolor{green!20} & .0103 \cellcolor{green!8} & .0103 \cellcolor{green!8} & .0054 \cellcolor{green!34} \\\texttt{RCV1-v2} & .0492 \cellcolor{red!35} & .0118$^{\dag\phantom{\dag}}$ \cellcolor{green!34} & .0181 \cellcolor{green!23} & .0165 \cellcolor{green!26} & .0214 \cellcolor{green!16} & .0214 \cellcolor{green!16} & \textbf{.0117} \cellcolor{green!35} \\\texttt{Mediamill} & .1713 \cellcolor{red!35} & .0212$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0204 \cellcolor{green!34} & \textbf{.0185} \cellcolor{green!35} & .0222 \cellcolor{green!33} & .0230 \cellcolor{green!32} & .0192 \cellcolor{green!34} \\\texttt{Bibtex} & .0358 \cellcolor{red!35} & .0102$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0112 \cellcolor{green!30} & .0111 \cellcolor{green!30} & .0116 \cellcolor{green!29} & .0119 \cellcolor{green!28} & \textbf{.0096} \cellcolor{green!35} \\\texttt{Corel5k} & .0582 \cellcolor{red!35} & .0076$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0082 \cellcolor{green!34} & .0088 \cellcolor{green!33} & \textbf{.0076} \cellcolor{green!35} & .0093 \cellcolor{green!32} & .0077 \cellcolor{green!34} \\\texttt{Delicious} & .1418 \cellcolor{red!35} & .0095$^{\ddag}$ \cellcolor{green!34} & .0102 \cellcolor{green!34} & \textbf{.0094} \cellcolor{green!35} & .0106 \cellcolor{green!34} & .0115 \cellcolor{green!33} & .0095 \cellcolor{green!34} \\\hline
\multicolumn{1}{|c|}{Average} & .0725 \cellcolor{red!35} & .0231 \cellcolor{green!34} & .0303 \cellcolor{green!24} & .0243 \cellcolor{green!33} & .0319 \cellcolor{green!22} & .0320 \cellcolor{green!22} & \textbf{.0229} \cellcolor{green!35} \\\multicolumn{1}{|c|}{Rank Average} &  5.8 \cellcolor{red!35} &  2.7 \cellcolor{green!25} &  4.1 \cellcolor{red!1} &  2.8 \cellcolor{green!24} &  4.8 \cellcolor{red!15} &  5.5 \cellcolor{red!28} & \textbf{2.3} \cellcolor{green!35} \\\hline

                \hline
                \end{tabular}
            

==> tables/old_acc_nocol.app.ae.tex <==

    \resizebox{\textwidth}{!}{%
            \begin{tabularx}{\textwidth}{@{}lYYYYYYYYYYYYY@{}} \toprule
             & \multicolumn{4}{c}{low shift} & \multicolumn{4}{c}{mid shift} & \multicolumn{4}{c}{high shift}\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
 & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLQ & \MLC\SEP\MLQ & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLQ & \MLC\SEP\MLQ & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLQ & \MLC\SEP\MLQ\\\midrule
\texttt{Corel5k} & .1525 & .2172 & .0090 & \textbf{.0090} & .1517 & .2151 & .0089 & \textbf{.0087} & .1505 & .2143 & .0097 & \textbf{.0097} \\
\texttt{Bibtex} & .0791 & .1283 & \textbf{.0162} & .0162 & .0699 & .1288 & .0116 & \textbf{.0113} & .0674 & .1296 & .0099 & \textbf{.0096} \\
\texttt{Birds} & .1565 & .1844 & .0369 & \textbf{.0309} & .1521 & .1615 & .0261 & \textbf{.0253} & .1570 & .1494 & .0228 & \textbf{.0227} \\
\texttt{Delicious} & .0873 & .0799 & \textbf{.0119} & .0120 & .0798 & .0711 & \textbf{.0110} & .0112 & .0648 & .0483 & \textbf{.0087} & .0093 \\
\texttt{Emotions} & .1281 & .0776 & \textbf{.0514} & .0547 & .1180 & .0830 & \textbf{.0503} & .0541 & .1414 & .1179 & \textbf{.0487} & .0815 \\
\texttt{Enron} & .1811 & .1969 & \textbf{.0207} & .0232 & .1845 & .2025 & \textbf{.0189} & .0212 & .2022 & .2319 & .0224 & \textbf{.0224} \\
\texttt{Genbase} & \textbf{.0015} & .0024 & .0033 & .0044 & \textbf{.0014} & .0022 & .0028 & .0042 & \textbf{.0011} & .0019 & .0024 & .0040 \\
\texttt{Mediamill} & .1348 & .1236 & \textbf{.0291} & .0295 & .0763 & .0711 & .0207 & \textbf{.0207} & .0484 & .0482 & .0165 & \textbf{.0164} \\
\texttt{Medical} & \textbf{.0167} & .0183 & .0201 & .0219 & .0204 & .0319 & .0226 & \textbf{.0201} & .0185 & .0285 & .0207 & \textbf{.0177} \\
\texttt{Ohsumed} & .0373 & .0340 & \textbf{.0246} & .0252 & .0314 & .0287 & .0221 & \textbf{.0218} & .0253 & .0240 & .0199 & \textbf{.0198} \\
rcv1 & .0292 & .0408 & \textbf{.0188} & .0216 & .0156 & .0325 & \textbf{.0119} & .0127 & .0132 & .0298 & \textbf{.0099} & .0099 \\
reuters21578 & .0384 & .0240 & \textbf{.0110} & .0114 & .0322 & .0207 & \textbf{.0073} & .0073 & .0307 & .0183 & .0047 & \textbf{.0046} \\
\texttt{Scene} & .0519 & .0420 & .0424 & \textbf{.0400} & .0597 & .0430 & .0424 & \textbf{.0419} & .0660 & \textbf{.0439} & .0568 & .0521 \\
\texttt{tmc2007\_500} & .1079 & .1047 & .0451 & \textbf{.0424} & .0525 & .0496 & .0272 & \textbf{.0251} & .0340 & .0324 & .0202 & \textbf{.0198} \\
\texttt{Yeast} & .2297 & .2405 & \textbf{.1131} & .1201 & .2010 & .2299 & \textbf{.0617} & .0659 & .1927 & .2241 & .0655 & \textbf{.0636} \\
\midrule
\multicolumn{1}{|c|}{Average} & .0944 \cellcolor{red!50} & .0933 \cellcolor{red!48} & \textbf{.0129} \cellcolor{green!50} & .0131 \cellcolor{green!49} & .0875 \cellcolor{red!18} & .1208 \cellcolor{red!50} & \textbf{.0140} \cellcolor{green!50} & .0141 \cellcolor{green!49} & .0425 \cellcolor{red!23} & .0535 \cellcolor{red!50} & .0116 \cellcolor{green!49} & \textbf{.0115} \cellcolor{green!50} \\

        \bottomrule
        \end{tabularx}%
        }
    

==> tables/old_cc_nocol.app.ae.tex <==

    \resizebox{\textwidth}{!}{%
            \begin{tabularx}{\textwidth}{@{}lYYYYYYYYYYYYY@{}} \toprule
             & \multicolumn{4}{c}{low shift} & \multicolumn{4}{c}{mid shift} & \multicolumn{4}{c}{high shift}\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
 & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLC & \MLC\SEP\MLQ & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLC & \MLC\SEP\MLQ & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLC & \MLC\SEP\MLQ\\\midrule
\texttt{Corel5k} & .0357 & .0092 & .0088 & \textbf{.0082} & .0358 & .0091 & .0088 & \textbf{.0080} & .0368 & .0092 & .0095 & \textbf{.0086} \\
\texttt{Bibtex} & .0179 & \textbf{.0139} & .0151 & .0158 & .0139 & \textbf{.0100} & .0101 & .0102 & .0126 & \textbf{.0081} & .0083 & .0083 \\
\texttt{Birds} & \textbf{.0290} & .0299 & .0358 & .0308 & .0249 & .0254 & .0284 & \textbf{.0247} & \textbf{.0218} & .0221 & .0255 & .0224 \\
\texttt{Delicious} & .1041 & .0119 & .0113 & \textbf{.0102} & .0929 & .0103 & .0103 & \textbf{.0093} & .0443 & \textbf{.0065} & .0074 & .0068 \\
\texttt{Emotions} & .0778 & .0772 & .0645 & \textbf{.0592} & .0795 & .0744 & .0674 & \textbf{.0616} & .1145 & .0952 & \textbf{.0534} & .0878 \\
\texttt{Enron} & .0254 & .0228 & \textbf{.0211} & .0226 & .0246 & .0206 & \textbf{.0192} & .0207 & .0242 & \textbf{.0186} & .0202 & .0200 \\
\texttt{Genbase} & .0004 & \textbf{.0003} & .0027 & .0026 & \textbf{.0003} & .0003 & .0022 & .0023 & \textbf{.0001} & .0003 & .0018 & .0020 \\
\texttt{Mediamill} & .1656 & .0451 & \textbf{.0293} & .0293 & .1454 & .0306 & .0209 & \textbf{.0202} & .1351 & .0221 & .0165 & \textbf{.0151} \\
\texttt{Medical} & .0185 & \textbf{.0148} & .0216 & .0164 & .0183 & \textbf{.0166} & .0198 & .0178 & .0171 & \textbf{.0160} & .0184 & .0170 \\
\texttt{Ohsumed} & .0442 & .0351 & .0304 & \textbf{.0274} & .0383 & .0293 & .0232 & \textbf{.0217} & .0345 & .0259 & .0196 & \textbf{.0191} \\
rcv1 & .0359 & .0250 & \textbf{.0198} & .0205 & .0226 & .0131 & .0126 & \textbf{.0119} & .0202 & .0095 & .0105 & \textbf{.0093} \\
reuters21578 & .0240 & .0093 & .0108 & \textbf{.0091} & .0105 & \textbf{.0063} & .0070 & .0064 & .0061 & \textbf{.0038} & .0046 & .0041 \\
\texttt{Scene} & .0794 & .0509 & .0499 & \textbf{.0368} & .0868 & .0445 & .0500 & \textbf{.0372} & .1245 & .0801 & .0592 & \textbf{.0420} \\
\texttt{tmc2007\_500} & .1090 & .0704 & .0544 & \textbf{.0505} & .0753 & .0399 & .0281 & \textbf{.0244} & .0610 & .0260 & .0203 & \textbf{.0191} \\
\texttt{Yeast} & .1544 & .1737 & .1154 & \textbf{.1140} & .1551 & .1215 & .0653 & \textbf{.0604} & .1782 & .1003 & .0693 & \textbf{.0634} \\
\midrule
\multicolumn{1}{|c|}{Average} & .0950 \cellcolor{red!50} & .0135 \cellcolor{green!47} & .0125 \cellcolor{green!48} & \textbf{.0115} \cellcolor{green!50} & .0423 \cellcolor{red!50} & .0162 \cellcolor{green!39} & .0140 \cellcolor{green!47} & \textbf{.0132} \cellcolor{green!50} & .0453 \cellcolor{red!50} & .0129 \cellcolor{green!43} & .0116 \cellcolor{green!47} & \textbf{.0107} \cellcolor{green!50} \\

        \bottomrule
        \end{tabularx}%
        }
    

==> tables/old_pacc_nocol.app.ae.tex <==

    \resizebox{\textwidth}{!}{%
            \begin{tabularx}{\textwidth}{@{}lYYYYYYYYYYYYY@{}} \toprule
             & \multicolumn{4}{c}{low shift} & \multicolumn{4}{c}{mid shift} & \multicolumn{4}{c}{high shift}\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
 & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLQ & \MLC\SEP\MLQ & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLQ & \MLC\SEP\MLQ & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLQ & \MLC\SEP\MLQ\\\midrule
\texttt{Corel5k} & .1539 & .2458 & \textbf{.0110} & .0118 & .1524 & .2472 & \textbf{.0108} & .0117 & .1580 & .2509 & \textbf{.0117} & .0122 \\
\texttt{Bibtex} & .0596 & .0944 & \textbf{.0158} & .0181 & .0339 & .0681 & \textbf{.0107} & .0122 & .0276 & .0581 & \textbf{.0088} & .0101 \\
\texttt{Birds} & .1311 & .2161 & .0333 & \textbf{.0314} & .1230 & .2029 & .0319 & \textbf{.0297} & .1283 & .1919 & .0305 & \textbf{.0290} \\
\texttt{Delicious} & .0636 & .0708 & \textbf{.0115} & .0117 & .0537 & .0637 & \textbf{.0105} & .0107 & .0340 & .0471 & .0084 & \textbf{.0083} \\
\texttt{Emotions} & .1399 & .1121 & \textbf{.0499} & .0587 & .1384 & .0929 & \textbf{.0506} & .0612 & .1569 & .1434 & \textbf{.0541} & .1067 \\
\texttt{Enron} & .1538 & .2672 & \textbf{.0243} & .0413 & .1439 & .2729 & \textbf{.0215} & .0397 & .1066 & .3025 & \textbf{.0178} & .0218 \\
\texttt{Genbase} & \textbf{.0019} & .0024 & .0033 & .0036 & \textbf{.0018} & .0023 & .0029 & .0032 & \textbf{.0016} & .0022 & .0025 & .0028 \\
\texttt{Mediamill} & .1273 & .0877 & .0277 & \textbf{.0268} & .0709 & .0508 & .0202 & \textbf{.0194} & .0441 & .0324 & .0160 & \textbf{.0154} \\
\texttt{Medical} & .0197 & .0277 & \textbf{.0182} & .0295 & .0440 & .0643 & \textbf{.0173} & .0194 & .0429 & .0593 & \textbf{.0175} & .0216 \\
\texttt{Ohsumed} & .0424 & .0307 & .0231 & \textbf{.0230} & .0327 & .0262 & .0204 & \textbf{.0202} & .0242 & .0224 & .0188 & \textbf{.0187} \\
rcv1 & .0492 & .0199 & \textbf{.0196} & .0205 & .0241 & \textbf{.0117} & .0122 & .0120 & .0218 & \textbf{.0092} & .0101 & .0094 \\
reuters21578 & .0509 & .0301 & \textbf{.0098} & .0128 & .0214 & .0161 & \textbf{.0068} & .0080 & .0079 & .0076 & \textbf{.0045} & .0047 \\
\texttt{Scene} & .0554 & \textbf{.0381} & .0428 & .0387 & .0621 & .0394 & .0475 & \textbf{.0364} & .0811 & .0447 & .0644 & \textbf{.0388} \\
\texttt{tmc2007\_500} & .0956 & .0743 & .0444 & \textbf{.0351} & .0520 & .0392 & .0249 & \textbf{.0230} & .0342 & .0293 & .0198 & \textbf{.0190} \\
\texttt{Yeast} & .2378 & .1453 & .1124 & \textbf{.1104} & .1815 & .1326 & \textbf{.0635} & .0645 & .1644 & .1433 & .0646 & \textbf{.0619} \\
\midrule
\multicolumn{1}{|c|}{Average} & .0737 \cellcolor{red!30} & .0886 \cellcolor{red!50} & \textbf{.0127} \cellcolor{green!50} & .0136 \cellcolor{green!48} & .0777 \cellcolor{red!14} & .1128 \cellcolor{red!50} & \textbf{.0144} \cellcolor{green!50} & .0155 \cellcolor{green!48} & .0339 \cellcolor{red!39} & .0366 \cellcolor{red!50} & .0115 \cellcolor{green!49} & \textbf{.0114} \cellcolor{green!50} \\

        \bottomrule
        \end{tabularx}%
        }
    

==> tables/old_pcc_nocol.app.ae.tex <==

    \resizebox{\textwidth}{!}{%
            \begin{tabularx}{\textwidth}{@{}lYYYYYYYYYYYYY@{}} \toprule
             & \multicolumn{4}{c}{low shift} & \multicolumn{4}{c}{mid shift} & \multicolumn{4}{c}{high shift}\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
 & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLQ & \MLC\SEP\MLQ & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLQ & \MLC\SEP\MLQ & \BC\SEP\BQ & \MLC\SEP\BQ & \BC\SEP\MLQ & \MLC\SEP\MLQ\\\midrule
Corel5k & .0579 & .0084 & .0097 & \textbf{.0077} & .0583 & .0082 & .0094 & \textbf{.0074} & .0593 & .0085 & .0099 & \textbf{.0080} \\
bibtex & .0425 & .0152 & \textbf{.0146} & .0151 & .0357 & .0103 & \textbf{.0097} & .0101 & .0340 & .0081 & \textbf{.0080} & .0082 \\
birds & .0372 & \textbf{.0271} & .0297 & .0287 & .0312 & \textbf{.0232} & .0248 & .0241 & .0290 & .0223 & \textbf{.0220} & .0222 \\
delicious & .1425 & .0096 & .0116 & \textbf{.0096} & .1284 & .0087 & .0105 & \textbf{.0087} & .0605 & .0062 & .0075 & \textbf{.0061} \\
emotions & .0535 & .0526 & \textbf{.0505} & .0558 & .0552 & .0542 & \textbf{.0499} & .0562 & .1052 & .1019 & \textbf{.0681} & .0881 \\
enron & .0357 & .0232 & .0204 & \textbf{.0201} & .0368 & .0205 & .0191 & \textbf{.0185} & .0457 & .0187 & .0203 & \textbf{.0181} \\
genbase & \textbf{.0011} & .0012 & .0037 & .0019 & .0011 & \textbf{.0010} & .0033 & .0015 & .0011 & \textbf{.0009} & .0029 & .0013 \\
mediamill & .1789 & .0362 & .0291 & \textbf{.0273} & .1709 & .0223 & .0210 & \textbf{.0192} & .1700 & .0157 & .0164 & \textbf{.0149} \\
medical & .0205 & .0169 & .0185 & \textbf{.0150} & \textbf{.0131} & .0161 & .0177 & .0170 & \textbf{.0140} & .0165 & .0160 & .0157 \\
ohsumed & .1142 & .0346 & \textbf{.0257} & .0261 & .1068 & .0241 & \textbf{.0202} & .0206 & .1021 & \textbf{.0166} & .0180 & .0183 \\
rcv1 & .0650 & .0233 & \textbf{.0182} & .0194 & .0492 & .0120 & .0115 & \textbf{.0113} & .0470 & .0090 & .0094 & \textbf{.0088} \\
reuters21578 & .0319 & .0112 & \textbf{.0089} & .0092 & .0216 & .0070 & .0065 & \textbf{.0064} & .0163 & \textbf{.0038} & .0043 & .0040 \\
scene & .0974 & .0487 & .0503 & \textbf{.0337} & .1027 & .0468 & .0553 & \textbf{.0365} & .1594 & .0981 & .0665 & \textbf{.0398} \\
tmc2007\_500 & .1375 & .0569 & .0505 & \textbf{.0434} & .1142 & .0274 & .0261 & \textbf{.0224} & .1038 & .0182 & .0198 & \textbf{.0181} \\
yeast & .1719 & .1109 & .1130 & \textbf{.1108} & .1825 & \textbf{.0620} & .0643 & .0631 & .2158 & .0756 & .0638 & \textbf{.0628} \\
\midrule
\multicolumn{1}{|c|}{Average} & .1302 \cellcolor{red!50} & .0112 \cellcolor{green!49} & .0127 \cellcolor{green!48} & \textbf{.0108} \cellcolor{green!50} & .0650 \cellcolor{red!50} & .0136 \cellcolor{green!48} & .0136 \cellcolor{green!48} & \textbf{.0126} \cellcolor{green!50} & .0705 \cellcolor{red!50} & .0106 \cellcolor{green!49} & .0110 \cellcolor{green!48} & \textbf{.0103} \cellcolor{green!50} \\

        \bottomrule
        \end{tabularx}%
        }
    

==> tables/simple.npp.ae.tex <==
\setlength\tabcolsep{1.5pt}
                \begin{tabular}{|l|cccc|cccc|cccc|cccc|cccc|} \cline{2-21}

            \multicolumn{1}{c|}{} & \multicolumn{4}{c|}{CC} & \multicolumn{4}{c|}{PCC} & \multicolumn{4}{c|}{ACC} & \multicolumn{4}{c|}{PACC} & \multicolumn{4}{c|}{SLD} \\\cline{2-21}
            \multicolumn{1}{c|}{} & \side{\bqbc} & \side{\bqmc} & \side{\mqbc} & \side{\mqmc\phantom{0}} & \side{\bqbc} & \side{\bqmc} & \side{\mqbc} & \side{\mqmc\phantom{0}} & \side{\bqbc} & \side{\bqmc} & \side{\mqbc} & \side{\mqmc\phantom{0}} & \side{\bqbc} & \side{\bqmc} & \side{\mqbc} & \side{\mqmc\phantom{0}} & \side{\bqbc} & \side{\bqmc} & \side{\mqbc} & \side{\mqmc\phantom{0}} \\\hline
\texttt{Emotions} & .0695 \cellcolor{green!21} & .0576 \cellcolor{green!26} & .0411 \cellcolor{green!32} & .0667 \cellcolor{green!22} & \textbf{.0335} \cellcolor{green!35} & .0337$^{\dag}$ \cellcolor{green!34} & .0554 \cellcolor{green!27} & .0447$^{\phantom{\ddag}}$ \cellcolor{green!30} & .1118 \cellcolor{green!6} & .1348 \cellcolor{red!1} & .0544 \cellcolor{green!27} & .0394 \cellcolor{green!32} & .1395 \cellcolor{red!3} & .0767 \cellcolor{green!19} & .0449 \cellcolor{green!30} & .0476 \cellcolor{green!29} & .2265 \cellcolor{red!35} & .0529 \cellcolor{green!27} & .0675 \cellcolor{green!22} & .0468 \cellcolor{green!30} \\\texttt{Scene} & .0753 \cellcolor{red!26} & .0544 \cellcolor{red!0} & .0449 \cellcolor{green!10} & .0324 \cellcolor{green!25} & .0828 \cellcolor{red!35} & \textbf{.0247}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0376 \cellcolor{green!19} & .0300$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0520 \cellcolor{green!2} & .0395 \cellcolor{green!17} & .0462 \cellcolor{green!9} & .0335 \cellcolor{green!24} & .0464 \cellcolor{green!8} & .0358 \cellcolor{green!21} & .0379 \cellcolor{green!19} & .0291 \cellcolor{green!29} & .0397 \cellcolor{green!16} & .0363 \cellcolor{green!21} & .0309 \cellcolor{green!27} & .0366 \cellcolor{green!20} \\\texttt{Yeast} & .1480 \cellcolor{red!1} & .1092 \cellcolor{green!10} & .0417 \cellcolor{green!31} & .0417 \cellcolor{green!31} & .1763 \cellcolor{red!10} & \textbf{.0300}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0374 \cellcolor{green!32} & .0384$^{\phantom{\ddag}}$ \cellcolor{green!32} & .1915 \cellcolor{red!15} & .1697 \cellcolor{red!8} & .0411 \cellcolor{green!31} & .0434 \cellcolor{green!30} & .1545 \cellcolor{red!3} & .1355 \cellcolor{green!2} & .0386 \cellcolor{green!32} & .0415 \cellcolor{green!31} & .2554 \cellcolor{red!35} & .0902 \cellcolor{green!16} & .0426 \cellcolor{green!31} & .0422 \cellcolor{green!31} \\\texttt{Birds} & .0225 \cellcolor{green!32} & .0250 \cellcolor{green!31} & .0200 \cellcolor{green!34} & .0210 \cellcolor{green!33} & .0288 \cellcolor{green!29} & .0214$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{.0187} \cellcolor{green!35} & .0222$^{\phantom{\ddag}}$ \cellcolor{green!33} & .1514 \cellcolor{red!35} & .1344 \cellcolor{red!26} & .0240 \cellcolor{green!32} & .0270 \cellcolor{green!30} & .1237 \cellcolor{red!20} & .1285 \cellcolor{red!22} & .0192 \cellcolor{green!34} & .0228 \cellcolor{green!32} & .0758 \cellcolor{green!4} & .0289 \cellcolor{green!29} & .0203 \cellcolor{green!34} & .0286 \cellcolor{green!29} \\\texttt{Genbase} & \textbf{.0003} \cellcolor{green!35} & .0006 \cellcolor{green!29} & .0017 \cellcolor{green!9} & .0007 \cellcolor{green!27} & .0011 \cellcolor{green!20} & .0005$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0023 \cellcolor{red!1} & .0007$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0014 \cellcolor{green!14} & .0007 \cellcolor{green!27} & .0037 \cellcolor{red!27} & .0006 \cellcolor{green!28} & .0018 \cellcolor{green!7} & .0010 \cellcolor{green!21} & .0041 \cellcolor{red!35} & .0015 \cellcolor{green!12} & .0011 \cellcolor{green!20} & .0003 \cellcolor{green!33} & .0039 \cellcolor{red!30} & .0005 \cellcolor{green!30} \\\texttt{Medical} & .0175 \cellcolor{green!19} & .0116 \cellcolor{green!34} & .0156 \cellcolor{green!23} & .0116 \cellcolor{green!34} & .0117 \cellcolor{green!34} & .0132$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0165 \cellcolor{green!21} & \textbf{.0113}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0208 \cellcolor{green!10} & .0301 \cellcolor{red!13} & .0164 \cellcolor{green!22} & .0163 \cellcolor{green!22} & .0385 \cellcolor{red!35} & .0256 \cellcolor{red!1} & .0154 \cellcolor{green!24} & .0142 \cellcolor{green!27} & .0231 \cellcolor{green!4} & .0130 \cellcolor{green!30} & .0166 \cellcolor{green!21} & .0127 \cellcolor{green!31} \\\texttt{tmc2007\_500} & .0686 \cellcolor{red!4} & .0288 \cellcolor{green!24} & .0189 \cellcolor{green!31} & .0187 \cellcolor{green!31} & .1103 \cellcolor{red!35} & \textbf{.0142}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0182 \cellcolor{green!32} & .0167$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0302 \cellcolor{green!23} & .0310 \cellcolor{green!22} & .0189 \cellcolor{green!31} & .0199 \cellcolor{green!30} & .0269 \cellcolor{green!25} & .0235 \cellcolor{green!28} & .0187 \cellcolor{green!31} & .0172 \cellcolor{green!32} & .0357 \cellcolor{green!19} & .0208 \cellcolor{green!30} & .0171 \cellcolor{green!32} & .0169 \cellcolor{green!33} \\\texttt{Ohsumed} & .0325 \cellcolor{green!20} & .0161 \cellcolor{green!33} & .0180 \cellcolor{green!31} & .0155 \cellcolor{green!33} & .1000 \cellcolor{red!35} & .0147$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0171 \cellcolor{green!32} & \textbf{.0142}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0234 \cellcolor{green!27} & .0229 \cellcolor{green!27} & .0185 \cellcolor{green!31} & .0165 \cellcolor{green!33} & .0210 \cellcolor{green!29} & .0202 \cellcolor{green!30} & .0181 \cellcolor{green!31} & .0158 \cellcolor{green!33} & .0281 \cellcolor{green!23} & .0163 \cellcolor{green!33} & .0164 \cellcolor{green!33} & .0162 \cellcolor{green!33} \\\texttt{Enron} & .0228 \cellcolor{green!31} & .0191 \cellcolor{green!33} & .0157 \cellcolor{green!34} & .0183 \cellcolor{green!33} & .0338 \cellcolor{green!26} & \textbf{.0145}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0155 \cellcolor{green!34} & .0174$^{\phantom{\ddag}}$ \cellcolor{green!33} & .1780 \cellcolor{red!35} & .0919 \cellcolor{green!1} & .0172 \cellcolor{green!33} & .0194 \cellcolor{green!32} & .1394 \cellcolor{red!18} & .1406 \cellcolor{red!18} & .0188 \cellcolor{green!33} & .0188 \cellcolor{green!33} & .0917 \cellcolor{green!1} & .0193 \cellcolor{green!32} & .0169 \cellcolor{green!33} & .0168 \cellcolor{green!34} \\\texttt{Reuters-21578} & .0058 \cellcolor{green!29} & \textbf{.0027} \cellcolor{green!35} & .0043 \cellcolor{green!32} & .0029 \cellcolor{green!34} & .0153 \cellcolor{green!14} & .0028$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0040 \cellcolor{green!32} & .0029$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0300 \cellcolor{red!10} & .0062 \cellcolor{green!29} & .0044 \cellcolor{green!32} & .0051 \cellcolor{green!31} & .0046 \cellcolor{green!31} & .0450 \cellcolor{red!35} & .0044 \cellcolor{green!32} & .0042 \cellcolor{green!32} & .0037 \cellcolor{green!33} & .0032 \cellcolor{green!34} & .0039 \cellcolor{green!33} & .0033 \cellcolor{green!34} \\\texttt{RCV1-v2} & .0177 \cellcolor{green!13} & \textbf{.0063} \cellcolor{green!35} & .0075 \cellcolor{green!32} & .0064 \cellcolor{green!34} & .0425 \cellcolor{red!35} & .0064$^{\ddag}$ \cellcolor{green!34} & .0070 \cellcolor{green!33} & .0064$^{\dag}$ \cellcolor{green!34} & .0093 \cellcolor{green!29} & .0196 \cellcolor{green!9} & .0073 \cellcolor{green!33} & .0080 \cellcolor{green!31} & .0099 \cellcolor{green!28} & .0084 \cellcolor{green!30} & .0073 \cellcolor{green!33} & .0070 \cellcolor{green!33} & .0085 \cellcolor{green!30} & .0075 \cellcolor{green!32} & .0068 \cellcolor{green!34} & .0073 \cellcolor{green!33} \\\texttt{Mediamill} & .1391 \cellcolor{red!12} & .0204 \cellcolor{green!31} & .0124 \cellcolor{green!34} & .0121 \cellcolor{green!34} & .1702 \cellcolor{red!23} & \textbf{.0109}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0121 \cellcolor{green!34} & .0118$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0451 \cellcolor{green!22} & .0398 \cellcolor{green!24} & .0131 \cellcolor{green!34} & .0124 \cellcolor{green!34} & .0372 \cellcolor{green!25} & .0391 \cellcolor{green!24} & .0127 \cellcolor{green!34} & .0127 \cellcolor{green!34} & .2008 \cellcolor{red!35} & .0193 \cellcolor{green!31} & .0119 \cellcolor{green!34} & .0117 \cellcolor{green!34} \\\texttt{Bibtex} & .0134 \cellcolor{green!29} & .0091 \cellcolor{green!34} & .0083 \cellcolor{green!34} & .0090 \cellcolor{green!34} & .0355 \cellcolor{green!8} & \textbf{.0081}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0082 \cellcolor{green!34} & .0083$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0676 \cellcolor{red!21} & .0809 \cellcolor{red!34} & .0092 \cellcolor{green!33} & .0095 \cellcolor{green!33} & .0283 \cellcolor{green!15} & .0180 \cellcolor{green!25} & .0088 \cellcolor{green!34} & .0090 \cellcolor{green!34} & .0817 \cellcolor{red!35} & .0098 \cellcolor{green!33} & .0087 \cellcolor{green!34} & .0096 \cellcolor{green!33} \\\texttt{Corel5k} & .0358 \cellcolor{green!20} & .0092 \cellcolor{green!33} & .0080 \cellcolor{green!34} & .0080 \cellcolor{green!34} & .0582 \cellcolor{green!9} & .0076$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0074 \cellcolor{green!34} & .0064$^{\phantom{\ddag}}$ \cellcolor{green!34} & .1518 \cellcolor{red!35} & .0175 \cellcolor{green!29} & .0081 \cellcolor{green!33} & \textbf{.0060} \cellcolor{green!35} & .1513 \cellcolor{red!34} & .1009 \cellcolor{red!10} & .0106 \cellcolor{green!32} & .0110 \cellcolor{green!32} & .1042 \cellcolor{red!12} & .0097 \cellcolor{green!33} & .0138 \cellcolor{green!31} & .0177 \cellcolor{green!29} \\\texttt{Delicious} & .1033 \cellcolor{red!15} & .0108 \cellcolor{green!33} & .0090 \cellcolor{green!34} & .0088 \cellcolor{green!34} & .1410 \cellcolor{red!35} & .0081$^{\dag}$ \cellcolor{green!34} & .0088 \cellcolor{green!34} & \textbf{.0079}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0803 \cellcolor{red!3} & .0523 \cellcolor{green!11} & .0092 \cellcolor{green!34} & .0085 \cellcolor{green!34} & .0531 \cellcolor{green!11} & .0398 \cellcolor{green!18} & .0089 \cellcolor{green!34} & .0087 \cellcolor{green!34} & .1353 \cellcolor{red!31} & .0133 \cellcolor{green!32} & .0089 \cellcolor{green!34} & .0096 \cellcolor{green!34} \\\hline
\multicolumn{1}{|c|}{Average} & .0353 \cellcolor{green!12} & .0262 \cellcolor{green!22} & .0195 \cellcolor{green!30} & .0214 \cellcolor{green!28} & .0385 \cellcolor{green!9} & \textbf{.0156}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0204 \cellcolor{green!29} & .0181$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0774 \cellcolor{red!35} & .0668 \cellcolor{red!22} & .0229 \cellcolor{green!26} & .0196 \cellcolor{green!30} & .0716 \cellcolor{red!28} & .0607 \cellcolor{red!16} & .0199 \cellcolor{green!30} & .0195 \cellcolor{green!30} & .0746 \cellcolor{red!31} & .0238 \cellcolor{green!25} & .0226 \cellcolor{green!27} & .0210 \cellcolor{green!28} \\\multicolumn{1}{|c|}{Rank Average} &  14.9 \cellcolor{red!23} &  9.1 \cellcolor{green!4} &  8.3 \cellcolor{green!7} &  6.0 \cellcolor{green!18} &  15.5 \cellcolor{red!25} & \textbf{2.5} \cellcolor{green!35} &  6.9 \cellcolor{green!14} &  3.6 \cellcolor{green!29} &  17.5 \cellcolor{red!35} &  16.2 \cellcolor{red!29} &  10.7 \cellcolor{red!3} &  8.9 \cellcolor{green!5} &  16.5 \cellcolor{red!30} &  14.9 \cellcolor{red!23} &  8.9 \cellcolor{green!4} &  7.7 \cellcolor{green!10} &  16.6 \cellcolor{red!30} &  9.7 \cellcolor{green!1} &  8.2 \cellcolor{green!8} &  7.5 \cellcolor{green!11} \\\hline

                \hline
                \end{tabular}
            
